Functional Linear Regression of Cumulative Distribution Functions

The estimation of cumulative distribution functions (CDF) is an important learning task with a great variety of downstream applications, such as risk assessments in predictions and decision making. In this paper, we study functional regression of contextual CDFs where each data point is sampled from a linear combination of context dependent CDF basis functions. We propose functional ridge-regression-based estimation methods that estimate CDFs accurately everywhere. In particular, given $n$ samples with $d$ basis functions, we show estimation error upper bounds of $\widetilde O(\sqrt{d/n})$ for fixed design, random design, and adversarial context cases. We also derive matching information theoretic lower bounds, establishing minimax optimality for CDF functional regression. Furthermore, we remove the burn-in time in the random design setting using an alternative penalized estimator. Then, we consider agnostic settings where there is a mismatch in the data generation process. We characterize the error of the proposed estimators in terms of the mismatched error, and show that the estimators are well-behaved under model mismatch. Moreover, to complete our study, we formalize infinite dimensional models where the parameter space is an infinite dimensional Hilbert space, and establish a self-normalized estimation error upper bound for this setting. Notably, the upper bound reduces to the $\widetilde O(\sqrt{d/n})$ bound when the parameter space is constrained to be $d$-dimensional. Our comprehensive numerical experiments validate the efficacy of our estimation methods in both synthetic and practical settings.

==> TMLR/Proof_sketches.tex <==
In this section, we provide the proof sketches of the main theoretical results in the paper. 

\subsection{Proof sketches of Theorem \ref{thm:upper_fixed} and Proposition \ref{prop:upper_fixed}} \label{sec:proof_sketch_upper_fixed}
The key idea in the proof of Theorem \ref{thm:upper_fixed} is to first notice that $\wh\theta_{\lambda}-\theta_*=U_n(\lambda)^{-1}W_n-U_n(\lambda)^{-1}(\lambda\theta_*)$, where $W_n:=\sum_{j=1}^n \int_S (\tI_{y^{(j)}}\Phi_j-\theta_*^{\top}\Phi_j\Phi_j)d\meas$. We next show that $\{\wb M_n\}_{n\ge 0}$ where
$\wb M_n:=\frac{\lambda^{d/2}}{\det(U_n(\lambda))^{1/2}}\exp\left(\frac{1}{2}\|W_n\|_{ U_n(\lambda)^{-1}}^2\right)$
is a super-martingale. \emph{Doob's maximal inequality} for super-martingales is then used in conjunction with some careful algebra to establish \eqref{eq:upperbound}. 
To prove Proposition \ref{prop:upper_fixed}, we use a vector \emph{Bernstein inequality} for bounded martingale difference sequences~\citep[Proposition 1.2]{10.1214/ECP.v17-2079} to show a high probability upper bound for $\|W_n\|$. Note that $U_N$ being positive definite implies that $U_n$ is positive definite for $n\ge N$. Since $\|\wh\theta-\theta_*\|_{U_n}=\|W_n\|_{U_n^{-1}}\le \|W_n\|/\sqrt{\mu_{\min}(U_n)}$, we establish \eqref{eq:upperbound_unreg}. 


\subsection{Proof sketches of Theorem \ref{thm:upper_random} and Proposition \ref{prop:upper_random}} \label{sec:proof_sketch_upper_random}
The main idea in the proofs of Theorem \ref{thm:upper_random} and Proposition \ref{prop:upper_random} is to establish a high probability lower bound on $\mu_{\min}(\Delta_n)$, where $\Delta_n:=\Sigma_n^{-\frac{1}{2}}\left(U_n-\Sigma_n\right)\Sigma_n^{-\frac{1}{2}}$. This can be achieved using the \emph{matrix Hoeffding's inequality} \cite[Theorem 1.3]{tropp2012user}. 
Then, we show that for any $\lambda\ge 0$, $\|\wh\theta_{\lambda}-\theta_*\|_{\Sigma_n}\le (1+\mu_{\min}\left(\Delta_n\right))^{-1/2}\|\wh\theta_{\lambda}-\theta_*\|_{U_n(\lambda)}$. 
For Theorem \ref{thm:upper_random}, we prove that $\mu_{\min}(U_n)\ge \mu_{\min}(\Sigma_n)(\mu_{\min}(\Delta_n)+1)$. Then, we can lower bound $\mu_{\min}(U_n)$ in \eqref{eq:upperbound_unreg} by a multiple of $\mu_{\min}(\Sigma_n)$ with high probability. Thus, \eqref{eq:upperbound_unreg_random} follows from \eqref{eq:upperbound_unreg} and the high probability lower bound on $\mu_{\min}(\Delta_n)$.
For Proposition \ref{prop:upper_random}, \eqref{eq:upperbound_random} follows from \eqref{eq:upperbound} and the high probability lower bound on $\mu_{\min}(\Delta_n)$.


\subsection{Proof sketch of Theorem \ref{thm:lower_fixed}} \label{sec:proof_sketch_lower_fixed}
In the proof of Theorem \ref{thm:lower_fixed}, we construct a family of $\Omega(a/\sqrt{d})$-packing subsets of $\Delta^{d-1}$ for $a\in(0,1)$ under $\ell^2$-distance. We then show that when $\phi_1,\dots,\phi_d$ are the \CDF{}s of $d$ Bernoulli distributions, for any $\theta^{(1)}\neq \theta^{(2)}$ in such a packing subset, the Kullback-Leibler (KL) divergence (see definition in Appendix \ref{sec:LB_fixed}) satisfies 
$$
D(P_{Y|x^{(j)};\theta^{(1)}}\|P_{Y|x^{(j)};\theta^{(2)}}) = O(a^2(1+\mu_{\min}(U_n))/d)
$$ 
for any $j\in[n]$. Since the above family of Bernoulli distributions is a subset of $\cP^d_{x^{1:n}}$, we are able to show that $\fR(\theta(\cP_{x^{1:n}}))=\Omega\big(\sqrt{d/(1+\mu_{\min}(U_n))}\big)$ using Fano's method and the aforementioned bound on KL divergence.


\subsection{Proof sketch of Theorem \ref{thm:upper_inf_dim}} \label{sec:proof_sketch_inf}
\input{TMLR/proof_sketch_inf}

==> TMLR/add_theory.tex <==
In this section, we present some additional theoretical results omitted in the main text.

\begin{corollary}[Self-normalized bound in fixed design setting] \label{coro:fixed_upper}
For an arbitrary probability measure $\meas$ on $S$ and an arbitrary sequence $\{x^{(j)}\}_{j\in\N}\in\X^\N$, assume that $y^{(j)}$ is sampled from $F(x^{(j)},\cdot)$ independently for each $j\in\N$ with $F$ defined in \eqref{eq:linear_model}. 
For any $\lambda>0$ and $\delta\in(0,1)$, with probability at least $1-\delta$, the estimator defined in \eqref{eq:estimator_general} satisfies \eqref{eq:upperbound} for all $n\in\N$.

If $U_N$ is positive definite for some fixed $N\in\N$, then for any $\delta\in(0,1)$ and $n\ge N$, with probability at least $1-\delta$, the estimator defined in \eqref{eq:estimator_general} with $\lambda=0$ satisfies \eqref{eq:upperbound_unreg}.
\end{corollary}
The proof of Corollary \ref{coro:fixed_upper} is inline with those of Theorem \ref{thm:upper_fixed} and Proposition \ref{prop:upper_fixed}. 
